Annolid: Annotate, Segment, and Track Anything You Need

Annolid is a deep learning-based software package designed for the segmentation, labeling, and tracking of research targets within video files, focusing primarily on animal behavior analysis. Based on state-of-the-art instance segmentation methods, Annolid now harnesses the Cutie video object segmentation model to achieve resilient, markerless tracking of multiple animals from single annotated frames, even in environments in which they may be partially or entirely concealed by environmental features or by one another. Our integration of Segment Anything and Grounding-DINO strategies additionally enables the automatic masking and segmentation of recognizable animals and objects by text command, removing the need for manual annotation. Annolid's comprehensive approach to object segmentation flexibly accommodates a broad spectrum of behavior analysis applications, enabling the classification of diverse behavioral states such as freezing, digging, pup huddling, and social interactions in addition to the tracking of animals and their body parts.

==> 02-related_works.tex <==
% This text has been copied to the appendix (appendix.tex) 
% This .tex file therefore is superfluous and can be deleted.

\section{Related Works}

\paragraph{Tracking-by-Detection Approaches}

Tracking-by-detection methodologies, as highlighted in studies such as \cite{kim2015multiple,tang2017multiple,bergmann2019tracking}, conventionally hinge upon the detection of segmentations within each frame, subsequently employing temporal propagation to link these per-frame segmentations. Notably, pose estimation-based multi-animal tracking packages like those elucidated in \cite{Lauer2022MultianimalPE,Pereira2022sleap} have garnered popularity. These solutions necessitate the labeling and training of networks to estimate poses, followed by the utilization of various techniques to identify and associate instances across frames. Moreover, these tools equip users with functionalities for manual correction and track merging, thereby enhancing the robustness and accuracy of the tracking process.


\paragraph{Universal Segmentation Tracking and Decoupled Video Segmentation}

In the realm of video object segmentation, conventional 'tracking-by-detection' methods hinge on image-level detections and short-term temporal tracking. However, recent advancements like SAM-PT \cite{rajivc2023segment} and DEVA \cite{cheng2023tracking} have introduced innovative strategies. The Segment Anything (SAM) framework, as demonstrated by Kirillov et al. \cite{kirillov2023segany}, underscores the efficacy and adaptability of large-scale training for universal image segmentation, thereby laying significant groundwork for open-world segmentation. Subsequent studies by Yang et al. \cite{yang2023track} and Cheng et al. \cite{cheng2023segment} extend SAM to video data by propagating masks generated by SAM using video object segmentation algorithms. Nevertheless, these approaches predominantly rely on single-frame segmentation and lack inherent denoising capability. To address this limitation, Cheng et al. \cite{cheng2023tracking} proposed an in-clip consensus approach.

\paragraph{Tracking by classifing Segmentation Masks}

idTracker.ai \cite{romero2019idtracker} employs threshold-based segmentation to isolate instances within frames, followed by classification networks to identify individual animals. Annolid \cite{yang2023automated} utilizes instance segmentation networks such as Mask R-CNN for segmentation and classification by assigning each instance its own class. SIPEC \cite{marks2022deep} utilizes an instance segmentation network to delineate animals within video frames and subsequently employs another network for animal identification, enabling the analysis of animal behavior in intricate environments using raw video data. SIPEC comprises four key modules: segmentation, identification, pose estimation, and behavioral classification. Notably, ~\cite{romero2019idtracker,marks2022deep} require more than 1000 labeled frames for training the identification networks.

\paragraph{Memory-Based VOS}

Semi-supervised Video Object Segmentation (VOS) involves directional propagation of information, leading many existing approaches to employ a feature memory representation for storing past features to segment future frames. This includes online learning methods that finetune a network on the first-frame segmentation for each video during inference. XMem~\cite{cheng2022xmem} leverages various memory types to enhance performance and efficiency, albeit facing challenges from noise introduced by low-level pixel matching. Cutie integrates memory reading techniques inspired by XMem~\cite{cheng2022xmem} and introduces an object reading mechanism. This integration empowers Cutie to achieve superior performance, particularly in demanding scenarios.


\paragraph{End-to-End Video Segmentation}

In the realm of semi-supervised Video Object Segmentation (VOS), the utilization of memory-based representations and Transformer-based methods has become pivotal for effectively segmenting future frames and conducting pixel matching with memory. A notable contribution in this domain is the introduction of Cutie~\cite{cheng2023putting}. Cutie presents an efficient object transformer framework that facilitates real-time processing by circumventing costly attention mechanisms. What sets Cutie apart is its ability to establish bi-directional communication between pixel-level and object-level features, thereby enhancing object-level reasoning. Unlike previous methods such as ISVOS~\cite{wang2023look}, Cutie adopts a fully-online approach that seamlessly segments subsequent frames within a video sequence. The bi-directional propagation mechanism used by Cutie unifies image segmentation and propagation models, enhancing video segmentation performance.One of the key strengths of Cutie lies in its integration of pixel memory and object memory representations, which enables the efficient retrieval and utilization of relevant information during segmentation tasks. Moreover, the incorporation of an object transformer enriches pixel features with object-level semantics, ensuring robust segmentation performance even in complex scenarios. Furthermore, Cutie's commitment to open-source principles enhances reproducibility and invites community contributions, thereby fostering collaborative advancements in the field of video object segmentation. Through its innovative design and practical implementation, Cutie represents a significant stride forward in the quest for efficient and effective video segmentation techniques.


\paragraph{Open-World Video Segmentation}

Recently, the introduction of a novel open-world video segmentation dataset, BURST \cite{athar2023burst}, marks a notable advancement in the field. BURST encompasses 482 object classes across diverse scenarios, evaluating open-world performance through separate metric computations for common classes (78, overlapping with COCO) and uncommon classes (404). The baseline method in BURST \cite{athar2023burst} predicts object proposals via an image instance segmentation model trained on COCO \cite{lin2014microsoft}, associating these proposals frame-by-frame using either box IoU or STCN \cite{cheng2021stcn}. OWTB \cite{liu2022opening} extends this by incorporating optical flow and pre-trained Re-ID features for proposal association. In contrast, Cutie approaches utilizes bi-directional propagation to generate segmentations, minimizing sensitivity to image segmentation errors. Another significant open-world video segmentation dataset, UVO \cite{du2021uvo}, predominantly focuses on human actions. These refined distinctions among approaches and datasets illuminate the nuances of video object segmentation and its diverse applications.


==> 10-how2install.tex <==

% Installing Annolid
\vspace{1 cm}
\section{Installing Annolid in a Conda Environment}

\subsection{Installing Conda}

If you don't have Conda installed on your system, you can install it by following these steps:

\subsection*{Windows:}

\begin{enumerate}
    \item \textbf{Download Anaconda Installer:}
        \begin{itemize}
            \item Go to the Anaconda website: \url{https://www.anaconda.com/products/distribution}.
            \item Download the appropriate version of Anaconda for Windows (32-bit or 64-bit).
        \end{itemize}
        
    \item \textbf{Run the Installer:}
        \begin{itemize}
            \item Once the installer is downloaded, double-click the executable file to launch the installer.
        \end{itemize}
        
    \item \textbf{Follow the Installation Wizard:}
        \begin{itemize}
            \item Follow the prompts in the installation wizard.
            \item Select the installation location and optionally add Anaconda to your PATH environment variable.
        \end{itemize}
        
    \item \textbf{Complete the Installation:}
        \begin{itemize}
            \item Click 'Next' and then 'Install' to begin the installation process.
            \item Once installed, you can access Conda via Anaconda Navigator or the Anaconda Prompt.
        \end{itemize}
        
    \item \textbf{Verification:}
        \begin{itemize}
            \item Open Anaconda Prompt from the Start menu.
            \item Type \texttt{conda --version} and press Enter. This command should display the Conda version installed.
        \end{itemize}
\end{enumerate}

\subsection*{Linux:}

\begin{enumerate}
    \item \textbf{Download Anaconda Installer:}
        \begin{itemize}
            \item Go to the Anaconda website: \url{https://www.anaconda.com/products/distribution}.
            \item Download the appropriate version of Anaconda for Linux.
        \end{itemize}
        
    \item \textbf{Open Terminal:}
        \begin{itemize}
            \item Open a terminal window on your Linux distribution.
        \end{itemize}
        
    \item \textbf{Navigate to the Download Directory:}
        \begin{itemize}
            \item Use the \texttt{cd} command to navigate to the directory where the Anaconda installer was downloaded.
        \end{itemize}
        
    \item \textbf{Run the Installer Script:}
        \begin{itemize}
            \item Use the following command to run the Anaconda installer script:
            \begin{verbatim}
            bash Anaconda3-<version>-Linux-x86_64.sh
            \end{verbatim}
            Replace \texttt{<version>} with the version number of Anaconda you downloaded.
        \end{itemize}
        
    \item \textbf{Follow the Installation Prompts:}
        \begin{itemize}
            \item Follow the prompts to agree to the license terms, select the installation location, and confirm the installation.
        \end{itemize}
        
    \item \textbf{Activate Installation:}
        \begin{itemize}
            \item After installation, source the \texttt{.bashrc} file to activate the changes:
            \begin{verbatim}
            source ~/.bashrc
            \end{verbatim}
        \end{itemize}
        
    \item \textbf{Verification:}
        \begin{itemize}
            \item Open a new terminal window.
            \item Type \texttt{conda --version} and press Enter. This command should display the Conda version installed.
        \end{itemize}
\end{enumerate}

\subsection*{macOS:}

\begin{enumerate}
    \item \textbf{Download Anaconda Installer:}
        \begin{itemize}
            \item Go to the Anaconda website: \url{https://www.anaconda.com/products/distribution}.
            \item Download the appropriate version of Anaconda for macOS.
        \end{itemize}
        
    \item \textbf{Open Terminal:}
        \begin{itemize}
            \item Launch Terminal from the Applications/Utilities folder or by searching in Spotlight.
        \end{itemize}
        
    \item \textbf{Navigate to the Download Directory:}
        \begin{itemize}
            \item Use the \texttt{cd} command to navigate to the directory where the Anaconda installer was downloaded.
        \end{itemize}
        
    \item \textbf{Run the Installer Script:}
        \begin{itemize}
            \item Use the following command to run the Anaconda installer script:
            \begin{verbatim}
            bash Anaconda3-<version>-MacOSX-x86_64.sh
            \end{verbatim}
            Replace \texttt{<version>} with the version number of Anaconda you downloaded.
        \end{itemize}
        
    \item \textbf{Follow the Installation Prompts:}
        \begin{itemize}
            \item Follow the prompts to agree to the license terms, select the installation location, and confirm the installation.
        \end{itemize}
        
    \item \textbf{Activate Installation:}
        \begin{itemize}
            \item After installation, source the \texttt{.bash\_profile} file to activate the changes:
            \begin{verbatim}
            source ~/.bash_profile
            \end{verbatim}
        \end{itemize}
        
    \item \textbf{Verification:}
        \begin{itemize}
            \item Open a new terminal window.
            \item Type \texttt{conda --version} and press Enter. This command should display the Conda version installed.
        \end{itemize}
\end{enumerate}


\section{Installation of Annolid on MacBook Air M2 Chip}
\begin{enumerate}
    \item Download the Conda installer for macOS from the official Conda website (\url{https://docs.conda.io/en/latest/miniconda.html}).
    \item Open a terminal window.
    \item Navigate to the directory where the Conda installer was downloaded.
    \item Run the following command to execute the installer:
    \begin{verbatim}
    bash Miniconda3-latest-MacOSX-x86_64.sh
    \end{verbatim}
    \item Follow the prompts to complete the installation. Make sure to agree to the license terms, and choose the installation location.
\end{enumerate}

To install Annolid on your MacBook Air M2 chip, follow these steps:
\subsection{Installing Annolid}

Once Conda is installed, you can proceed with installing Annolid:

\begin{enumerate}
    \item Open a terminal window.
    \item Check the version of Conda installed by running:
    \begin{verbatim}
    conda -V
    \end{verbatim}
    \item Create a new Conda environment for Annolid:
    \begin{verbatim}
    conda create -n annolid python=3.11
    \end{verbatim}
    \item Activate the newly created environment:
    \begin{verbatim}
    conda activate annolid
    \end{verbatim}
    \item Clone the Annolid repository and its submodules using Git:
    \begin{verbatim}
    git clone --recurse-submodules https://github.com/healthonrails/annolid.git
    \end{verbatim}
    \item Change into the Annolid directory:
    \begin{verbatim}
    cd annolid
    \end{verbatim}
    \item Install Annolid in editable mode using pip:
    \begin{verbatim}
    pip install -e .
    \end{verbatim}
    \item Run Annolid:
    \begin{verbatim}
    annolid
    \end{verbatim}
    \item To deactivate the Annolid environment and return to the base environment, run:
    \begin{verbatim}
    conda deactivate
    \end{verbatim}
\end{enumerate}

\subsection{Removing Annolid}

If you wish to remove the Annolid environment from your system, you can do so using the following command:

\begin{verbatim}
conda env remove --name annolid
\end{verbatim}

This command will remove the Annolid environment and all its associated packages.

To check the list of Conda environments on your system, you can run:
\begin{verbatim}
conda info --envs
\end{verbatim}

\section{Installing Conda on Windows 10}
\date{\today}
\begin{enumerate}
    \item \textbf{Download Anaconda}: Visit the \href{https://www.anaconda.com/products/distribution}{Anaconda download page} and download the appropriate installer for Windows.
    
    \item \textbf{Run the Installer}: Double-click the downloaded installer to launch the installation process.
    
    \item \textbf{Follow the Installation Wizard}: Follow the prompts in the installation wizard, selecting appropriate options. It's recommended to add Anaconda to your system PATH.
    
    \item \textbf{Complete Installation}: Once the installation is complete, close the installer.
\end{enumerate}

\section{Installing CUDA and PyTorch (if using GPU)}

\begin{enumerate}
    \item \textbf{Verify CUDA Version}: Open Command Prompt and run the following command to check the CUDA version:
    \begin{verbatim}
        nvidia-smi
    \end{verbatim}
    Ensure that the CUDA version is compatible with the version of PyTorch you intend to install.
    
    \item \textbf{Install PyTorch with CUDA support}: If your CUDA version is compatible, you can install PyTorch with CUDA support using Conda. Run the following command:
    \begin{verbatim}
    conda install pytorch==2.2.0 torchvision==0.17.0 \
     torchaudio==2.2.0 pytorch-cuda=12.1 -c pytorch -c nvidia
    \end{verbatim}
    Replace the version numbers and CUDA version with your desired versions if necessary.
\end{enumerate}

\section{Installing Annolid}

\begin{enumerate}
    \item \textbf{Open Command Prompt}: Press \texttt{Win + R} to open the Run dialog, type \texttt{cmd}, and press Enter.
    
    \item \textbf{Create a Conda Environment for Annolid}:
    \begin{verbatim}
        conda create -n annolid-env python=3.11
    \end{verbatim}
    
    \item \textbf{Activate the Environment}:
    \begin{verbatim}
        conda activate annolid-env
    \end{verbatim}
    
    \item \textbf{Clone the Annolid Repository}:
    \begin{verbatim}
        git clone --recurse-submodules https://github.com/healthonrails/annolid.git
    \end{verbatim}
    
    \item \textbf{Navigate to the Annolid Directory}:
    \begin{verbatim}
        cd annolid
    \end{verbatim}
    
    \item \textbf{Install Annolid Using pip}:
    \begin{verbatim}
        pip install -e .
    \end{verbatim}

    \item \textbf{Launch Annolid}:
    \begin{verbatim}
     annolid
    \end{verbatim} 
    
    \item \textbf{Remove the Conda Environment (Optional)}:
    \begin{verbatim}
        conda env remove --name annolid-env
    \end{verbatim}
\end{enumerate}

\section{Tips for Installation}

\begin{itemize}
    \item \textbf{Environment Management}: Conda allows you to create separate environments for different projects, which helps in managing dependencies.
    
    \item \textbf{Python Version}: Annolid requires Python 3.11. Make sure to specify the correct Python version when creating the Conda environment.
    
    \item \textbf{Git Installation}: Before cloning the Annolid repository, make sure you have Git installed on your system.
    
    \item \textbf{Submodules}: Annolid relies on Git submodules. Use the \texttt{--recurse-submodules} flag while cloning the repository to ensure all necessary dependencies are downloaded.
\end{itemize}

By following these steps, you should be able to install Annolid on your Windows 10 system successfully. Make sure to activate the Conda environment whenever you want to work with Annolid by running \texttt{conda activate annolid-env} in the Command Prompt.


\section{Installing Annolid on Ubuntu 20.04}

\subsection{Installing Conda on Ubuntu 20.04}

\begin{enumerate}
    \item \textbf{Download Miniconda}: Visit the \href{https://docs.conda.io/en/latest/miniconda.html}{Miniconda website} and download the appropriate installer script for Linux.
    
    \item \textbf{Run the Installer Script}: Open a terminal and navigate to the directory where the Miniconda installer script is downloaded. Run the following command to execute the script:
    \begin{verbatim}
        bash Miniconda3-latest-Linux-x86_64.sh
    \end{verbatim}
    Follow the prompts in the installer to complete the installation. You may need to close and reopen the terminal after installation.
    Replace \texttt{myenv} with your desired environment name and specify the Python version if necessary.
\end{enumerate}

\subsection{Installing CUDA and PyTorch (if using GPU)}

\begin{enumerate}
    \item \textbf{Verify CUDA Version}: Open a terminal and run the following command to check the CUDA version:
    \begin{verbatim}
        nvidia-smi
    \end{verbatim}
    Ensure that the CUDA version is compatible with the version of PyTorch you intend to install.
    
    \item \textbf{Install PyTorch with CUDA support}: If your CUDA version is compatible, you can install PyTorch with CUDA support using Conda. Run the following command:
    \begin{verbatim}
    conda install pytorch==2.2.0 torchvision==0.17.0 \
     torchaudio==2.2.0 cudatoolkit=12.1 -c pytorch -c nvidia
    \end{verbatim}
    Replace the version numbers and CUDA version with your desired versions if necessary.
\end{enumerate}

\subsection{Installing Annolid}

\begin{enumerate}
    \item \textbf{Open a Terminal}: Press \texttt{Ctrl + Alt + T} to open a terminal window.
    
    \item \textbf{Create a Conda Environment for Annolid}:
    \begin{verbatim}
        conda create -n annolid-env python=3.11
    \end{verbatim}
    
    \item \textbf{Activate the Environment}:
    \begin{verbatim}
        conda activate annolid-env
    \end{verbatim}
    
    \item \textbf{Clone the Annolid Repository}:
    \begin{verbatim}
        git clone --recurse-submodules https://github.com/healthonrails/annolid.git
    \end{verbatim}
    
    \item \textbf{Navigate to the Annolid Directory}:
    \begin{verbatim}
        cd annolid
    \end{verbatim}
    
    \item \textbf{Install Annolid Using pip}:
    \begin{verbatim}
        pip install -e .
    \end{verbatim}
    \item \textbf{Launch Annolid}:
    \begin{verbatim}
     annolid
    \end{verbatim} 

    \item \textbf{Remove the Conda Environment (Optional)}:
    \begin{verbatim}
        conda env remove --name annolid-env
    \end{verbatim}
\end{enumerate}

\subsection{Tips for Installation}

\begin{itemize}
    \item \textbf{Environment Management}: Conda allows you to create separate environments for different projects, which helps in managing dependencies.
    
    \item \textbf{Python Version}: Annolid requires Python 3.11. Make sure to specify the correct Python version when creating the Conda environment.
    
    \item \textbf{Git Installation}: Ensure that Git is installed on your Ubuntu system. You can install it using the following command:
    \begin{verbatim}
        sudo apt update
        sudo apt install git
    \end{verbatim}
    
    \item \textbf{Submodules}: Annolid relies on Git submodules. Use the \texttt{--recurse-submodules} flag while cloning the repository to ensure all necessary dependencies are downloaded.
\end{itemize}

By following these steps, you should be able to install Annolid on your Ubuntu 20.04 system successfully. Make sure to activate the Conda environment whenever you want to work with Annolid by running \texttt{conda activate annolid-env} in the terminal.



==> 11-how2use.tex <==

\section{Using Annolid: A Step-by-Step Guide}

This guide will walk you through using Annolid to track objects in your videos. Each step is designed to be easy to follow, ensuring you get the most out of the software.

\subsection{Step 1: Open Your Video and Label Instances}

Start by opening Annolid and loading the video you want to work with. You can do this by clicking on the video icon in the toolbar or selecting "Open Video" from the menu.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\textwidth]{imgs/annolid/AI_polygon.png}
  \caption{Opening a Video in Annolid}
  \label{fig:open_video_annolid}
\end{figure}

Once the video is loaded, right-click to bring up the menu and choose "AI-Polygon" Click on the object you want to track, and Annolid will generate a polygon around it. You can adjust the polygon as needed and assign a unique identifier to each instance. 
Clicking plus CMD or CTRL will bring up a pop-up dialog for you to enter the information for each instance. When you are done with labeling, use CMD or CTRL + S or click the save button in the toolbar to save the labeled instances to a JSON file.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\textwidth]{imgs/annolid/click_save_polygon.png}
  \caption{Labeling Instances in Annolid}
  \label{fig:label_first_frame_annolid}
\end{figure}

\subsection{Step 2: Predict and Track Based on the First Frame}

After labeling the first frame, it's time to start tracking! Click on the "Pred" button to initiate the tracking process. Annolid will run its model inference in the background, and you can start checking the predictions by navigating through the frames.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\textwidth]{imgs/annolid/stop_prediction_and_correction.png}
  \caption{Starting Tracking in Annolid}
  \label{fig:tracking_prediciton}
\end{figure}

\subsection{Step 3: Stop and Verify the Predictions}

If you notice any inaccuracies in the predictions, you can stop the process by clicking the red "Stop" button. Annolid allows you to delete predictions from the next frame onwards and make corrections as needed.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\textwidth]{imgs/annolid/delete_prediction_from_next_frame.png}
  \caption{Stopping and Correcting Predictions in Annolid}
  \label{fig:stop_and_predict}
\end{figure}

\subsection{Step 4: Finalize the Predictions}

Once you're satisfied with the tracking, you can finalize the predictions. Annolid makes it easy to review and complete the tracking task, ensuring accuracy and reliability.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{imgs/annolid/check_and_finish_prediction.png}
    \caption{Completing the Tracking Task in Annolid}
    \label{fig:complete_the_tracking_task}
  \end{figure}

  Congratulations! You've successfully used Annolid to track objects in your videos. Feel free to close the program or continue exploring its other features. 

  Your tracking results will be saved to a folder with the same name as the video. It will contain all the JSON files following the convention 
  'video\_name\_frame\_number.json', as well as 'video\_name\_tracking.csv' and 'video\_name\_tracked.csv' files. Please refer to Tables \ref{tab:motion_data} and \ref{tab:tracking_reulst_with_mask} for details.

==> tabs/tab-matd.tex <==
% Table is superfluous, I think.  Omitted.
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Video}      & \textbf{Corrections}  & \textbf{Frames} & \textbf{every\_mem} & \textbf{Process} \\ \midrule
Two mice  & 0                     & 2559              & 1                    & Auto-label "mouse"              \\
Dancing birds  & 0                     & 359              & 1                    & Auto-label "bird"             \\
Five goldfish            & 2                     & 655              & 1                    & Label "fish", predict, correct occlusions            \\
Two polar bears   & 2                     & 959              & 1                    & Auto-label "polar bear", predict, correct occlusions   \\ 

\bottomrule
\end{tabular}
